Galaxy-galaxy lensing with the DES-CMASS catalogue: measurement and constraints on the galaxy-matter cross-correlation

The DMASS sample is a photometric sample from the DES Year 1 data set designed to replicate the properties of the CMASS sample from BOSS, in support of a joint analysis of DES and BOSS beyond the small overlapping area. In this paper, we present the measurement of galaxy-galaxy lensing using the DMASS sample as gravitational lenses in the DES Y1 imaging data. We test a number of potential systematics that can bias the galaxy-galaxy lensing signal, including those from shear estimation, photometric redshifts, and observing conditions. After careful systematic tests, we obtain a highly significant detection of the galaxy-galaxy lensing signal, with total $S/N=25.7$. With the measured signal, we assess the feasibility of using DMASS as gravitational lenses equivalent to CMASS, by estimating the galaxy-matter cross-correlation coefficient $r_{\rm cc}$. By jointly fitting the galaxy-galaxy lensing measurement with the galaxy clustering measurement from CMASS, we obtain $r_{\rm cc}=1.09^{+0.12}_{-0.11}$ for the scale cut of $4~h^{-1}{\rm Mpc}$ and $r_{\rm cc}=1.06^{+0.13}_{-0.12}$ for $12~h^{-1}{\rm Mpc}$ in fixed cosmology. By adding the angular galaxy clustering of DMASS, we obtain $r_{\rm cc}=1.06\pm 0.10$ for the scale cut of $4~h^{-1}{\rm Mpc}$ and $r_{\rm cc}=1.03\pm 0.11$ for $12~h^{-1}{\rm Mpc}$. The resulting values of $r_{\rm cc}$ indicate that the lensing signal of DMASS is statistically consistent with the one that would have been measured if CMASS had populated the DES region within the given statistical uncertainty. The measurement of galaxy-galaxy lensing presented in this paper will serve as part of the data vector for the forthcoming cosmology analysis in preparation.

==> authorlist_mnras.tex <==
% Author list file generated with: mkauthlist 1.2.4 
% mkauthlist -f -j mnras --sort-builder DES-2020-0531_author_list_sorted.csv authorlist_mnras.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
S.~Lee,$^{1}$
M.~A.~Troxel,$^{1}$
A.~Choi,$^{2}$
J.~Elvin-Poole,$^{2,3}$
C.~Hirata,$^{2,3}$
K.~Honscheid,$^{2,3}$
E.~M.~Huff,$^{4}$
N.~MacCrann,$^{5}$
A.~J.~Ross,$^{2}$
T.~F.~Eifler,$^{6,4}$
C.~Chang,$^{7,8}$
R.~Miquel,$^{9,10}$
Y.~Omori,$^{11}$
J.~Prat,$^{7}$
G.~M.~Bernstein,$^{12}$
C.~Davis,$^{11}$
J.~DeRose,$^{13,14}$
M.~Gatti,$^{12}$
M.~M.~Rau,$^{15}$
S.~Samuroff,$^{15}$
C.~S{\'a}nchez,$^{12}$
P.~Vielzeuf,$^{10}$
J.~Zuntz,$^{16}$
M.~Aguena,$^{17,18}$
S.~Allam,$^{19}$
A.~Amon,$^{11}$
F.~Andrade-Oliveira,$^{20,18}$
E.~Bertin,$^{21,22}$
D.~Brooks,$^{23}$
D.~L.~Burke,$^{11,24}$
A.~Carnero~Rosell,$^{25,18,26}$
M.~Carrasco~Kind,$^{27,28}$
J.~Carretero,$^{10}$
F.~J.~Castander,$^{29,30}$
R.~Cawthon,$^{31}$
C.~Conselice,$^{32,33}$
M.~Costanzi,$^{34,35,36}$
L.~N.~da Costa,$^{18,37}$
M.~E.~S.~Pereira,$^{38}$
J.~De~Vicente,$^{39}$
S.~Desai,$^{40}$
H.~T.~Diehl,$^{19}$
J.~P.~Dietrich,$^{41}$
P.~Doel,$^{23}$
S.~Everett,$^{14}$
A.~E.~Evrard,$^{42,38}$
I.~Ferrero,$^{43}$
B.~Flaugher,$^{19}$
P.~Fosalba,$^{29,30}$
J.~Frieman,$^{19,8}$
J.~Garc\'ia-Bellido,$^{44}$
E.~Gaztanaga,$^{29,30}$
D.~W.~Gerdes,$^{42,38}$
T.~Giannantonio,$^{45,46}$
D.~Gruen,$^{47,11,24}$
R.~A.~Gruendl,$^{27,28}$
J.~Gschwend,$^{18,37}$
G.~Gutierrez,$^{19}$
W.~G.~Hartley,$^{48}$
S.~R.~Hinton,$^{49}$
D.~L.~Hollowood,$^{14}$
B.~Hoyle,$^{41,50}$
D.~Huterer,$^{38}$
D.~J.~James,$^{51}$
K.~Kuehn,$^{52,53}$
N.~Kuropatkin,$^{19}$
O.~Lahav,$^{23}$
M.~Lima,$^{17,18}$
M.~A.~G.~Maia,$^{18,37}$
M.~March,$^{12}$
J.~L.~Marshall,$^{54}$
F.~Menanteau,$^{27,28}$
J.~J.~Mohr,$^{41,50}$
R.~Morgan,$^{31}$
A.~Palmese,$^{19,8}$
F.~Paz-Chinch\'{o}n,$^{27,45}$
A.~Pieres,$^{18,37}$
A.~A.~Plazas~Malag\'on,$^{55}$
A.~Roodman,$^{11,24}$
E.~Sanchez,$^{39}$
V.~Scarpine,$^{19}$
M.~Schubnell,$^{38}$
S.~Serrano,$^{29,30}$
I.~Sevilla-Noarbe,$^{39}$
E.~Sheldon,$^{56}$
M.~Smith,$^{57}$
E.~Suchyta,$^{58}$
M.~E.~C.~Swanson,$^{27}$
G.~Tarle,$^{38}$
D.~Thomas,$^{59}$
C.~To,$^{47,11,24}$
T.~N.~Varga,$^{50,60}$
and J.~Weller$^{50,60}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{2}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{3}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{4}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{5}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{6}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{7}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{8}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{9}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{10}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{11}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{12}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{13}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{14}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{15}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{16}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
$^{17}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{18}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{19}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{20}$ Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil\\
$^{21}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{22}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{23}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{24}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{25}$ Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{26}$ Universidad de La Laguna, Dpto. Astrofisica, E-38206 La Laguna, Tenerife, Spain\\
$^{27}$ Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{28}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{29}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{30}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{31}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{32}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{33}$ University of Nottingham, School of Physics and Astronomy, Nottingham NG7 2RD, UK\\
$^{34}$ Astronomy Unit, Department of Physics, University of Trieste, via Tiepolo 11, I-34131 Trieste, Italy\\
$^{35}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{36}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{37}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{38}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{39}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{40}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{41}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{42}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{43}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{44}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{45}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{46}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{47}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{48}$ Department of Astronomy, University of Geneva, ch. d'\'Ecogia 16, CH-1290 Versoix, Switzerland\\
$^{49}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{50}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{51}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{52}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{53}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{54}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{55}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{56}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{57}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{58}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{59}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{60}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
}
}

